Formulation of Supersymmetry on a Lattice as a Representation of a Deformed Superalgebra

The lattice superalgebra of the link approach is shown to satisfy a Hopf algebraic supersymmetry where the difference operator is introduced as a momentum operator. The breakdown of the Leibniz rule for the lattice difference operator is accommodated as a coproduct operation of (quasi)triangular Hopf algebra and the associated field theory is consistently defined as a braided quantum field theory. Algebraic formulation of path integral is perturbatively defined and Ward-Takahashi identity can be derived on the lattice. The claimed inconsistency of the link approach leading to the ordering ambiguity for a product of fields is solved by introducing an almost trivial braiding structure corresponding to the triangular structure of the Hopf algebraic superalgebra. This could be seen as a generalization of spin and statistics relation on the lattice. From the consistency of this braiding structure of fields a grading nature for the momentum operator is required.

==> abbrv.tex <==
%% This is file 'abbrv.tex'.
%% ----- Identification -----
\NeedsTeXFormat{LaTeX2e}
\ProvidesFile{abbrv.tex}[2008/11/01]

\newlength{\brcktH}
%% ----------------------------------------
%% Abbreviations
%% ----------------------------------------

\newcommand{\naive}{na\"{\i}ve\ }
\newcommand{\Naive}{Na\"{\i}ve\ }
\newcommand{\naively}{na\"{\i}vely\ }
\newcommand{\Kahler}{K\"ahler\ }
\newcommand{\role}{r\^ole\ }

%% ----------------------------------------
%% Lattice operators
%% ----------------------------------------

\newcommand{\muhat}{\ensuremath{\hat{\mu}}}
\newcommand{\nuhat}{\ensuremath{\hat{\nu}}}
\newcommand{\Ql}{\ensuremath{Q^\MR{lat}}}
\newcommand{\Dl}{\ensuremath{D^\MR{lat}}}
\newcommand{\Qtl}{\ensuremath{\tilde{Q}^\MR{lat}}}
\newcommand{\Dtl}{\ensuremath{\tilde{D}^\MR{lat}}}
\newcommand{\Qlh}{\ensuremath{\hat{Q}^\MR{lat}}}
\newcommand{\Dlh}{\ensuremath{\hat{D}^\MR{lat}}}
\newcommand{\Qtlh}{\ensuremath{\hat{\tilde{Q}}^\MR{lat}}}
\newcommand{\Dtlh}{\ensuremath{\hat{\tilde{D}}^\MR{lat}}}
\newcommand{\Qlc}{\ensuremath{\MC{Q}^\MR{lat}}}
\newcommand{\Qlch}{\ensuremath{\hat{\MC{Q}}^\MR{lat}}}
\newcommand{\Dlc}{\ensuremath{\MC{D}^\MR{lat}}}
\newcommand{\Dlch}{\ensuremath{\hat{\MC{D}}^\MR{lat}}}
\newcommand{\Qco}{\ensuremath{\MC{Q}^\MR{op}}}
\newcommand{\Pl}{\ensuremath{P^\MR{lat}}}
\newcommand{\Plc}{\ensuremath{\MC{P}^\MR{lat}}}
\newcommand{\Plh}{\ensuremath{\hat{P}^\MR{lat}}}
\newcommand{\Plch}{\ensuremath{\hat{\MC{P}}^\MR{lat}}}
\newcommand{\delh}{\ensuremath{\hat{\del}}}
\newcommand{\dell}{\ensuremath{\del^\MR{lat}}}
\newcommand{\dellh}{\ensuremath{\hat{\del}^\MR{lat}}}
\newcommand{\deltal}{\ensuremath{\delta^\MR{lat}}}
\newcommand{\deltalh}{\ensuremath{\hat{\delta}^\MR{lat}}}
\newcommand{\Th}{\ensuremath{\hat{T}}}
\newcommand{\Qlcth}{\ensuremath{\hat{\tilde{\MC{Q}}}^\MR{lat}}}
\newcommand{\Dlcth}{\ensuremath{\hat{\tilde{\MC{D}}}^\MR{lat}}}
\newcommand{\shift}{\ensuremath{T}}
\newcommand{\clock}{\ensuremath{\Omega}}
\newcommand{\fn}{\ensuremath{\MC{F}}}
\newcommand{\statfn}{\ensuremath{(-1)^{\fn}}}

\newcommand{\at}{\ensuremath{\tilde{a}}}

%% ----------------------------------------
%% Fields
%% ----------------------------------------

\newcommand{\Vph}{\ensuremath{\hat{\Vp}}}
\newcommand{\chih}{\ensuremath{\hat{\chi}}}
\newcommand{\phih}{\ensuremath{\hat{\phi}}}
\newcommand{\Phih}{\ensuremath{\hat{\Phi}}}
\newcommand{\Phib}{\ensuremath{\bar{\Phi}}}
\newcommand{\Phibh}{\ensuremath{\hat{\bar{\Phi}}}}
\newcommand{\phit}{\ensuremath{\tilde{\phi}}}
\newcommand{\phith}{\ensuremath{\hat{\tilde{\phi}}}}
\newcommand{\thetah}{\ensuremath{\hat{\theta}}}
\newcommand{\thetab}{\ensuremath{\bar{\theta}}}
\newcommand{\thetabh}{\ensuremath{\hat{\bar{\theta}}}}
\newcommand{\thetat}{\ensuremath{\tilde{\theta}}}
\newcommand{\thetath}{\ensuremath{\hat{\tilde{\theta}}}}
\newcommand{\psih}{\ensuremath{\hat{\psi}}}
\newcommand{\Psih}{\ensuremath{\hat{\Psi}}}
\newcommand{\psit}{\ensuremath{\tilde{\psi}}}
\newcommand{\psith}{\ensuremath{\hat{\tilde{\psi}}}}
\newcommand{\sigmah}{\ensuremath{\hat{\sigma}}}
\newcommand{\sigmat}{\ensuremath{\tilde{\sigma}}}
\newcommand{\sigmath}{\ensuremath{\hat{\tilde{\sigma}}}}
\newcommand{\Dh}{\ensuremath{\hat{D}}}
\newcommand{\Fh}{\ensuremath{\hat{F}}}

%% ----------------------------------------
%% Hopf algebra
%% ----------------------------------------

\newcommand{\product}{\ensuremath{m}}
\newcommand{\opprod}{\ensuremath{\operatorname{\cdot}}}
\newcommand{\ncprod}{\ensuremath{\ast}}
\newcommand{\fprod}{\ensuremath{\cdot}}
\newcommand{\Lat}{\ensuremath{\MBB{L}}}
\newcommand{\Ind}{\ensuremath{\MBB{I}}}
\newcommand{\Xe}{\ensuremath{X_\MR{e}}}
\newcommand{\Xo}{\ensuremath{X_\MR{o}}}
\newcommand{\U}{\ensuremath{\MC{U}}}
\newcommand{\A}{\ensuremath{\MC{A}}}
\newcommand{\R}{\ensuremath{\MC{R}}}
\newcommand{\F}{\ensuremath{\MC{F}}}
\newcommand{\cocycle}{\ensuremath{\chi}}
\newcommand{\Xh}{\ensuremath{\hat{X}}}
\newcommand{\al}{\ensuremath{a^\MR{l}}}
\newcommand{\ar}{\ensuremath{a^\MR{r}}}
\newcommand{\Ll}{\ensuremath{L^\MR{l}{}}}
\newcommand{\Lr}{\ensuremath{L^\MR{r}{}}}
\newcommand{\Llr}{\ensuremath{L^\MR{l,r}{}}}
\newcommand{\Lp}{\ensuremath{L_{+}}}
\newcommand{\Tl}{\ensuremath{\overleftarrow{T}}}
\newcommand{\counit}{\ensuremath{\epsilon}}
\newcommand{\coproduct}{\ensuremath{\Delta}}
\newcommand{\antipode}{\ensuremath{S}}
\newcommand{\ot}{\ensuremath{\otimes}}
\newcommand{\ev}{\ensuremath{\operatorname{ev}}}
\newcommand{\coev}{\ensuremath{\operatorname{coev}}}
\newcommand{\diff}{\ensuremath{\operatorname{diff}}}
\newcommand{\fd}[1]{\ensuremath{\frac{\delta}{\delta#1}}}
\newcommand{\pd}[1]{\ensuremath{\frac{\del}{\del#1}}}
\newcommand{\Zz}{\ensuremath{Z^{(0)}}}
\newcommand{\Sint}{\ensuremath{S_\MR{int}}}

%% ----------------------------------------
%% General macros
%% ----------------------------------------

\newcommand{\DS}{\displaystyle}
\newcommand{\empbrckt}[1]{\settoheight{\brcktH}{#1}%
	\rule[-\brcktH/4]{0pt}{\brcktH}\null}

\newcommand{\MR}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\MC}[1]{\ensuremath{\mathcal{#1}}}
\newcommand{\MB}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\MBB}[1]{\ensuremath{\mathbb{#1}}}
\newcommand{\bs}[1]{{\ensuremath{\boldsymbol{#1}}}}

\newcommand{\del}{\ensuremath{\partial}}
\newcommand{\Order}[1]{\ensuremath{\operatorname{\mathcal{O}}(#1)}}
\newcommand{\RA}{\ensuremath{\rightarrow}}
\newcommand{\act}{\ensuremath{\operatorname{\rhd}}}
\newcommand{\Tr}{\ensuremath{\operatorname{Tr}}}
\newcommand{\Ad}{\ensuremath{\operatorname{Ad}}}
\newcommand{\ad}{\ensuremath{\operatorname{ad}}}
\newcommand{\Ve}{\ensuremath{\varepsilon}}
\newcommand{\Vp}{\ensuremath{\varphi}}
\newcommand{\IE}{\ensuremath{\text{\quad i.e.\quad}}}
\newcommand{\ST}{\ensuremath{\text{\quad s.t.\quad}}}
\newcommand{\OR}{\ensuremath{\text{\quad or\quad}}}
\newcommand{\AND}{\ensuremath{\text{\quad and\quad}}}
\newcommand{\lhs}{\ensuremath{(\text{l.h.s.})}}
\newcommand{\rhs}{\ensuremath{(\text{r.h.s.})}}
\newcommand{\Lin}{\ensuremath{\operatorname{Lin}}}

\newcommand{\id}{\ensuremath{\operatorname{id}}}
\newcommand{\vid}{%
 {\settowidth\unitlength{\ensuremath{\boldsymbol{1}}}%.3em
  \begin{picture}(1,1)
  \put(0.385,0){\makebox[0pt]{\ensuremath{\mathrm{1}}}}
  \put(0.615,0){\makebox[0pt]{\ensuremath{\mathrm{l}}}}
  \end{picture}}}
\newcommand{\lowest}[1][1]{%
	\ifcase#1%
		\ensuremath{\ |}%
	\or%
		\ensuremath{\ \big|}%
	\or%
		\ensuremath{\ \Big|}%
	\or%
		\ensuremath{\ \bigg|}%
	\or%
		\ensuremath{\ \Bibb|}%
	\fi}
\newcommand{\stat}[1]{%
	{\ensuremath{|#1|}}}
\newcommand{\fid}{\ensuremath{\mathbf{1}}}

% End of file 'abbrv.tex'.

